The Random Magnetic Field of the Milky Way

We constrain the large-scale isotropic random component of the Galactic magnetic field using the Planck reconstruction of the 408 MHz synchrotron sky. Our analysis simultaneously fits the random-field structure, the synchrotron contributions of the coherent field and local foregrounds, and isotropic and dipolar offsets. A new element of the analysis is the use of excess polarized emission at 30 GHz to model local foregrounds, allowing us to retain 97% of the sky without absorbing these structures into Galaxy-wide features of the magnetic field. Across variations in the coherent-field model, cosmic-ray electron distribution, sky mask, and field profile, we consistently find that the dominant random-field component is a vertically compact disk with a local rms strength of about 4 $\mu$G and a 1/e scale height of approximately 1 kpc, substantially thinner than in most previous models. An annular enhancement in the inner Galaxy improves the fit to the data, whereas we find no evidence for either a large-scale spiral pattern or a thick random-field disk. The fits also yield an intensity monopole of 4-7 K, whose possible origin we discuss. We quantify the implications of the inferred random field for the angular smearing of ultrahigh-energy cosmic rays. Compared with previous models, the sky-median smearing angle is smaller by up to a factor of 1.7, and by up to 2.4 in individual directions.

==> style.tex <==
% some colors
\definecolor{rossoCP3}{cmyk}{0,.88,.77,.40}
\definecolor{darkBlue}{rgb}{0, 0, 0.8}

% underbrace
\usepackage{tikz}
\usetikzlibrary{decorations.pathreplacing, calligraphy}
\makeatletter
\newsavebox\ub@box
\def\underbrace#1{\@ifnextchar_{\tikz@@ub{#1}}{\tikz@@ub{#1}_{}}}
\def\tikz@@ub#1_#2{%
  \sbox\ub@box{\(\displaystyle#1\)}%
  \pgfmathsetlengthmacro\ub@len{max(\the\wd\ub@box,1.2em)}%
  \pgfmathsetlengthmacro\ub@amp{min(4pt,0.25*\ub@len)}%
  \tikz[baseline=(a.base)]{%
    \node[inner sep=1pt] (a) {\usebox\ub@box};
    \draw[line cap=round, decorate,
          decoration={calligraphic brace, amplitude=\ub@amp}]
      ([xshift=0.5*\ub@len]a.south) --
        node[below, inner sep=7pt] {\(\scriptstyle#2\)}
      ([xshift=-0.5*\ub@len]a.south);}}
\makeatother

% footnotes
\makeatletter
\renewcommand{\@makefntext}[1]{%
  \noindent\llap{\@makefnmark\enspace}#1%
}
\makeatother

\hypersetup{
  bookmarks=true,         % show bookmarks bar?
  bookmarksopen=true,     % open bookmarks
  bookmarksopenlevel=1,
  unicode=false,          % non-Latin characters in Acrobat’s bookmarks
  pdftoolbar=true,        % show Acrobat’s toolbar?
  pdfmenubar=true,        % show Acrobat’s menu?
  colorlinks=true,        % false: boxed links; true: colored links
  linkcolor=darkBlue,     % color of internal links
  citecolor=darkBlue,     % color of links to bibliography
  filecolor=darkBlue,     % color of file links
  urlcolor=darkBlue       % color of external links
}

\makeatletter
\def\ApjSectionpenalty{\@M}
\makeatother

\DeclareFontFamily{U}{BOONDOX-calo}{\skewchar\font=45 }
\DeclareFontShape{U}{BOONDOX-calo}{m}{n}{
  <-> s*[1.05] BOONDOX-r-calo}{}
\DeclareFontShape{U}{BOONDOX-calo}{b}{n}{
  <-> s*[1.05] BOONDOX-b-calo}{}
\DeclareMathAlphabet{\mathcalboondox}{U}{BOONDOX-calo}{m}{n}
\SetMathAlphabet{\mathcalboondox}{bold}{U}{BOONDOX-calo}{b}{n}
\DeclareMathAlphabet{\mathbcalboondox}{U}{BOONDOX-calo}{b}{n}

